Combining Monte-Carlo and Hyper-heuristic methods for the Multi-mode Resource-constrained Multi-project Scheduling Problem

Multi-mode resource and precedence-constrained project scheduling is a well-known challenging real-world optimisation problem. An important variant of the problem requires scheduling of activities for multiple projects considering availability of local and global resources while respecting a range of constraints. A critical aspect of the benchmarks addressed in this paper is that the primary objective is to minimise the sum of the project completion times, with the usual makespan minimisation as a secondary objective. We observe that this leads to an expected different overall structure of good solutions and discuss the effects this has on the algorithm design. This paper presents a carefully designed hybrid of Monte-Carlo tree search, novel neighbourhood moves, memetic algorithms, and hyper-heuristic methods. The implementation is also engineered to increase the speed with which iterations are performed, and to exploit the computing power of multicore machines. Empirical evaluation shows that the resulting information-sharing multi-component algorithm significantly outperforms other solvers on a set of "hidden" instances, i.e. instances not available at the algorithm design phase.

==> background.tex <==
\section{Background}
\label{sec:background}

\subsection{Project Scheduling}
Project scheduling has been of interest to academics as well as practitioners. Solving such a problem requires scheduling of interrelated jobs (activities), potentially each using or sharing  scarce resources, subject to a set of constraints. There is a variety of project scheduling problems and there are many relevant surveys on this topic in the literature \cite{Brucker1999,Herroelen1998,Herroelen2005,Linet1995,Hartmann2010,Weglarz2011}. A well-known benchmark of project scheduling problems is provided in \cite{Kolisch1997}. Project scheduling can be broadly grouped under the following main categories; single-mode, multi-mode, resource-constrained single-mode and resource-constrained multi-mode. Single-mode project scheduling with resource constraints has been proven to be NP-hard \cite{Blazewicz1983}, hence the problem dealt with in this study is also a complex problem to solve.
\subsubsection{Solution Methods for resource-constrained multi-mode project scheduling}
In designing an algorithm, there are two `natural' representations to be used in the search for an assignment of activities to times:

\begin{itemize}

\item[] \textbf{Schedule-based:} A direct representation using the assignment times of activities.

\item[] \textbf{Sequence-based:} This is based on a selecting a total order on all the activities.
Given such a sequence then a time schedule is constructed by taking the activities one at a time in the order of the sequence and placing each one at the earliest time that it will go in the schedule.

\end{itemize}

The recent proposed solution methodologies for resource-constrained multi-mode project scheduling problem range from exact approaches, such as, MILP \cite{Kyriakidis2012}, to metaheuristics, such as, differential evolution \cite{Damak:2009}, estimation of distribution algorithms \cite{Wang2012}, evolutionary algorithms \cite{Elloumi2010}. Multi-project variant of this problem can still be reduced to a single project.

The schedule-based representation is perhaps the most natural for a mathematical programming approach, but we believe that it could make the search process difficult for a metaheuristic method, in particular, generating a feasible solution at each step could become more challenging.
Hence, we preferred the sequence-based representation, since it provides the ease of producing schedules that are both feasible and for which no activity can be moved to an earlier time without moving some other activities.


\subsection{Search Methodologies}
While solving computationally difficult problems, exact methods often fail, particularly when the problem instance size increases. Then alternative approaches, such as, heuristics, metaheuristics or hyper-heuristics are preferred in problem solving.

\subsubsection{Monte Carlo Search Trees}
Monte-Carlo Tree Search (MCTS) methods \cite{BrowneEtal2012:MCTS}.

\subsubsection{Memetic Algorithms}
A genetic algorithm is a metaheuristic which simulates evolution for problem solving.  A population of candidate solutions is evolved to obtain a high quality solution at the end of the whole process. Mate/parent selection, recombination, mutation and replacement are the main phases of an evolutionary algorithm. The candidate solutions, referred to as individuals or chromosomes go through an evolutionary cycle (each referred to as generation) passing through those phases. First, parent individuals are selected from the population, often favoring the high quality solutions, then they are recombined, producing new individuals which are exposed to mutation perturbing those new solutions further. The usefulness of recombination is still under debate in the research community (e.g., in favour \cite{Doerr:2008} and against \cite{mitchell93}). Replacement operator decides which individuals will survive to the next generation. A memetic algorithm hybridises a genetic algorithm with local search which is applied after mutation on the new individuals \cite{Moscato:89,Moscato:92}. A memetic algorithm is tailored for the problem dealt with \cite{Neri:12}. Sometimes a given algorithm could fail while dealing with even an unseen instance.

\subsubsection{Hyper-heuristics}
There is a growing interest towards self configuring/tuning automated heuristic approaches, such as, hyper-heuristics. A hyper-heuristic is a search methodology which explores the space of heuristics (i.e., move operators) rather than the solutions in problem solving \cite{burkeSurvey}. There are two common types of hyper-heuristics in the literature \cite{Burke:09}:
%
{\em selection} methodologies that choose/mix a heuristic from a set of preset low-level heuristics and attempt to control those heuristics during the search process; and {\em generation} methodologies that aim to build new heuristics from a set of given components.
%
%In this study, we provide an approach based on a selection type of hyper-heuristic.
The  main components of an iterative selection hyper-heuristic are  {\em heuristic selection}  and {\em move acceptance} methods.
At each step, an input solution is modified using a selected heuristic from a set of low-level heuristics. Then the quality of  new  and input solution is compared using the move acceptance method to decide whether to accept or reject the new solution. More on different types of hyper-heuristics, their components and application domains can be found in \cite{burkeSurvey,Burke:et,Ross:05,Ozcan:08}.

In this study, we hybridise different solution methods, for example, we use a hyper-heuristic as a local search component of a memetic algorithm for an improved performance to solve a resource-constrained multi-mode multi-project scheduling problem.


==> construction-fig-mid.tex <==
\begin{figure*}[bth]

\begin{subfigure}[b]{0.46\textwidth}
\begin{tikzpicture}
\begin{axis}[
	xlabel={$C_1$},
	ylabel={$C_2$},
	axis equal,
	width=\textwidth,
	height=5cm,
	grid=major
]
\addplot coordinates{
	(19,	41)
	(20,	41)
	(21,	41)
	(22,	41)
	(23,	41)
	(24,	40)
};
\end{axis}
\end{tikzpicture}
\caption{MISTA instance A-2}
\label{fig:TPD-mid-A2}
\end{subfigure}
%
\hspace{0.08\textwidth}
%
\begin{subfigure}[b]{0.46\textwidth}
\begin{tikzpicture}
\begin{axis}[
	xlabel={$C_1$},
	ylabel={$C_2$},
	axis equal,
	width=\textwidth,
	height=5cm,
	grid=major
]
\addplot coordinates{
	(58, 40)
	(59, 32)
	(60, 31)
	(61, 31)
	(62, 31)
	(63, 31)
	(64, 30)
	(65, 30)
	(66, 30)
	(67, 30)
	(68, 29)
	(69, 29)
	(70, 29)
	(71, 29)
	(72, 26)
};
\end{axis}
\end{tikzpicture}
\caption{Reduced/tightened instance.}
\label{fig:TPD-mid-artificial}
\end{subfigure}
\caption{Tradefoff between the two project completions times, 
% for a variety of generated schedules, 
on two medium-sized instances.}
\label{fig:TPD-mid}
\end{figure*}


==> mrcmpsp.tex <==
\section{MRCMPSP}

TODO Daniel: Add a couple of sentences about this section.

\input{problem-description}
\input{problem-analysis}
\input{test-instances}


==> problem-analysis.tex <==
\subsection{Problem Analysis}
\label{sec:problem-analysis}


